Minimal bandwidth $\mathbb{C}^*$-actions on generalized Grassmannians

The bandwidth of a $\mathbb{C}^*$-action of a polarized pair $(X,L)$ is a natural measure of its complexity. In this paper we study $\mathbb{C}^*$-actions on rational homogeneous spaces, determining which provide minimal bandwidth. We prove that the minimal bandwidth is linked to the smallest coefficient of the fundamental weight, in a base of simple roots, which describes the variety as a marked Dynkin diagram. As a direct application of the results we study the Chow ring of the Cayley plane $\mathrm{E}_6(6)$.

==> main.tex <==
%!TEX root = MinBW.tex

\section{Minimal bandwidth $\C^*$-actions on RH varieties}\label{sec:proof}


